Employ Multimodal Machine Learning for Content quality analysis

The task of identifying high-quality content becomes increasingly important, and it can improve overall reading time and CTR(click-through rate estimates). Generalizes quality analysis only focused on single Modal,such as image or text,but in today's mainstream media sites a lot of information is presented in graphic form.In this paper we propose a MultiModal quality recognition approach for the quality score. First we use two feature extractors,one for image and another for the text. After that we use an Siamese Network with the rank loss as the optimization objective.Compare with other approach,our approach get a more accuracy result.

==> tips/1.tex <==
abstract





